Airtnt: Fair Exchange Payment for Outsourced Secure Enclave Computations

We present Airtnt, a novel scheme that enables users with CPUs that support Trusted Execution Environments (TEEs) and remote attestation to rent out computing time on secure enclaves to untrusted users. Airtnt makes use of the attestation capabilities of TEEs and smart contracts on distributed ledgers to guarantee the fair exchange of the payment and the result of an execution. Airtnt makes use of off-chain payment channels to allow requesters to pay executing nodes for intermediate "snapshots" of the state of an execution. Effectively, this step-by-step "compute-payment" cycle realises untrusted pay-as-you-go micropayments for computation. Neither the requester nor the executing node can walk away and incur monetary loss to the other party. This also allows requesters to continue executions on other executing nodes if the original executing node becomes unavailable or goes offline.

==> sections/discussion.tex <==
\section{Discussion and Limitations}

\subsection{Multi-hop Payment Channels}

\subsection{Limitations of Intel SGX}
In term of performances, Intel SGX introduces memory limitations and performance overhead. Intel SGX limits the enclave memory to 128 MB; this limitation comes from the BIOS, and sets and upper bound to the input size that the executors can process simultaneously. It is however technically possible to extend that limit by editing the paging support~\cite{sgx2}. The performance overhead results from accessing the encrypted memory in an enclave and from the additional effort associated with entering and exiting an enclave. As shown in \Cref{implementation}, minimizing the number of accesses to the enclave significantly increases performances.

On the security side, relying on Intel SGX requires trust into Intel, as debated by many works~\cite{sgx_bad1, jackson2017trust, sgx_bad2, sgx_bad3}.

==> sections/issues.tex <==
\section{Open Issues}
\subsection{How to do flexible payments where the computational cost is not known in advance, for example because it is a function of the input.} 
During the meeting we sketched a solution including periodic payments ala payment channels. The executing node sends the results chunk by chunk and expects being paid by each chunk. Payment channels do not charge any fee per transaction, so it allows to decrease the cost and build the trust between both parties. \alberto{The above does not answer the question; I think we should simply say that the function creator is responsible of creating a payment policy (i.e., either a fixed amount, or a price as function of the input).}

TODO: Discuss with Patrick

\textbf{Problems:}
\begin{itemize}
\item Establishing a channel requires a transaction and involve locking some founds as a deposit. We want any node to be able to claim and execute the task, so establishing a channel in advance is not scalable. If we establish it after the execution node is chosen - it increases the delay. 
\item Maybe introducing many-to-many payments channel can be a thing?
\end{itemize}

\subsection{How to make the system suitable for delay sensitive tasks?}
Using smart contracts or making a payment/deposit require transaction. It takes few minutes for a transaction to be confirmed. We should think of more lightweight solutions allowing to submit small (and thus cheap), delay-sensitive tasks. 

\subsection{How to submit the results so that the blockchain can verify it?}
Results might be too large so we can’t just add them to the blockchain. Sending the results through TEE's TLS connection is not always an option, because i) blockchain can't verify it ii) in many scenario the result should be send to a 3rd party (and not to the requestor). We could think of using some public storage such as IPFS. The results would be publicly accessible, but signed and encrypted, so that anyone (including the blockchain) could verify their integrity, but cannot access the content. 

\subsection{Reputation System}
Blockchain is used in the system not as a source of trust, but as a marketplace for payment handling and a decentralized reputation system for executors (executors that finish their computation successfully push the proof to the blockchain and earn reputation points).
\todo[inline]{This is also something we will probably need to mention upfront, as it's different to many existing approaches.}

